On Multiplicative Linear Logic, Modality and Quantum Circuits

A logical system derived from linear logic and called QMLL is introduced and shown able to capture all unitary quantum circuits. Conversely, any proof is shown to compute, through a concrete GoI interpretation, some quantum circuits. The system QMLL, which enjoys cut-elimination, is obtained by endowing multiplicative linear logic with a quantum modality.

==> eptcsdata.tex <==
\providecommand{\firstpage}{55}
\providecommand{\publicationstatus}{Bart Jacobs, Peter Selinger, and Bas Spitters (Eds.):\\ 8th International Workshop on Quantum Physics and Logic (QPL 2011)\\
EPTCS 95, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.95.6}{10.4204/EPTCS.95.6}}
\pdfoutput=1

